Real-time Egocentric Gesture Recognition on Mobile Head Mounted Displays

Mobile virtual reality (VR) head mounted displays (HMD) have become popular among consumers in recent years. In this work, we demonstrate real-time egocentric hand gesture detection and localization on mobile HMDs. Our main contributions are: 1) A novel mixed-reality data collection tool to automatic annotate bounding boxes and gesture labels; 2) The largest-to-date egocentric hand gesture and bounding box dataset with more than 400,000 annotated frames; 3) A neural network that runs real time on modern mobile CPUs, and achieves higher than 76% precision on gesture recognition across 8 classes.

==> discussion.tex <==
\section{Applications to Other Data Colllection Tasks}
Our \textit{label as you go} approach can be adapted to other data 
collection tasks. Below are a few potential extensions of our approach:

\begin{itemize}[nosep]
  \item \textbf{Keypoint Annotation}: We
    could ask users to follow point trajectories with specific keypoints on
    tracked objects. For example, we could ask users to follow a trajectory with
    their fingers to create a fingertip dataset. 
  \item \textbf{Segmentation Mask Annotation}: We could
    utilize synthetically rendered masks of objects in different poses, and ask
    users to align them to objects in real-life with a smartphone app. This
    could potentially help generate much larger segmentation mask datasets.
\end{itemize}

Note that our approach is not limited to the mobile mixed reality setup. Mixed
reality provides natural \textit{hand}-eye coordination and is particularly effective
when gathering hand datasets. The same approach can
also be adapted and deployed on regular smartphones, where users could be asked to move their
phone such that the object in the viewfinder fits into the rendered target.


==> references.tex <==
\section*{References}

References follow the acknowledgments. Use unnumbered first-level
heading for the references. Any choice of citation style is acceptable
as long as you are consistent. It is permissible to reduce the font
size to \verb+small+ (9 point) when listing the references. {\bf
  Remember that you can go over 8 pages as long as the subsequent ones contain
  \emph{only} cited references.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms
for connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and
T.K.\ Leen (eds.), {\it Advances in Neural Information Processing
  Systems 7}, pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS:
  Exploring Realistic Neural Models with the GEneral NEural SImulation
  System.}  New York: TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of
learning and recall at excitatory recurrent synapses and cholinergic
modulation in rat hippocampal region CA3. {\it Journal of
  Neuroscience} {\bf 15}(7):5249-5262.



